DinTucker: Scaling up Gaussian process models on multidimensional arrays with billions of elements

Infinite Tucker Decomposition (InfTucker) and random function prior models, as nonparametric Bayesian models on infinite exchangeable arrays, are more powerful models than widely-used multilinear factorization methods including Tucker and PARAFAC decomposition, (partly) due to their capability of modeling nonlinear relationships between array elements. Despite their great predictive performance and sound theoretical foundations, they cannot handle massive data due to a prohibitively high training time. To overcome this limitation, we present Distributed Infinite Tucker (DINTUCKER), a large-scale nonlinear tensor decomposition algorithm on MAPREDUCE. While maintaining the predictive accuracy of InfTucker, it is scalable on massive data. DINTUCKER is based on a new hierarchical Bayesian model that enables local training of InfTucker on subarrays and information integration from all local training results. We use distributed stochastic gradient descent, coupled with variational inference, to train this model. We apply DINTUCKER to multidimensional arrays with billions of elements from applications in the "Read the Web" project (Carlson et al., 2010) and in information security and compare it with the state-of-the-art large-scale tensor decomposition method, GigaTensor. On both datasets, DINTUCKER achieves significantly higher prediction accuracy with less computational time.

==> algo2.tex <==
\subsection{Algorithm complexity}
\cmt{
In this section, we present a distributed inference procedure of \ours over MapReduce framework. Since updating   $\{\tUcal_n\}_{n=1}^N$ are independent given $\Ucal$, we can issue $N$ Mapper tasks, where each Mapper process a group of sub-arrays and perform SGD to update the corresponding $\tUcal_n$.
The estimating of $\Ucal$ needs to aggregate all the group-specific latent factors and we can assign a Reduce task correspondingly. The whole procedure is listed in Algorithm \ref{alg:dintucker}.
}
The time complexity of \InfTucker is $O(\sum_{k=1}^K m_k^3 + m_km)$ where $m_k$ is the dimension of the $k$-th mode and $m=\prod_{k=1}^K m_k$. It includes the eigen-decomposition of covariance matrix over each mode and tensor-matrix multiplications. For \ours,  suppose each sub-array has $\mhat_k$ dimensions in $k$-th mode, then the time complexity to process one sub-array is $O(\sum_{k=1}^K \mhat_k^3 + \mhat_k\mhat)$ where $\mhat = \prod_{k=1}^K\mhat_k$. If we set the dimension in each mode to be the same, the time complexity is $O(\mhat^(1+\frac{1}{K}))$. Suppose we have $L$ sub-arrays in total and $N$ computational nodes, the total time complexity is $O(\frac{L}{N}\mhat^(1+\frac{1}{K}))$. 
%If we take $\mhat_k = \frac{\max({m_k}_{k=1}^K)}{} $

For the space complexity, \InfTucker requires to store the whole multidimensional data in memory as well as the covariance matrix in each mode, \ie $O(m + \sum_{k=1}^K m_k^2)$, which is not feasible in large data. \ours only needs to store one sub-array in each MAPPER node and latent factor matrices in both MAPPER nodes and REDUCER node, thus, the space complexity is $O(\mhat + \sum_{k=1}^K r_k \mhat_k)$ where $r_k$ is the dimension of latent factors in mode $k$. Compared to \InfTucker, it is a huge reduction of the space and \ours is therefore able to deal with large scaled data.


\begin{algorithm}                      % enter the algorithm environment
\caption{SGD($\Scal_n$, T, $\eta$, $\Ucal$)}          % give the algorithm a caption
\label{alg:sgd}                           % and a label for \ref{} commands later in the document
\begin{algorithmic}                    % enter the algorithmic environment
    \STATE Random shuffle sub-arrays in $\Scal_n$.
    \STATE Initialize $\tUcal_n$ with $\Ucal$.
    \FOR {t=1 \TO $T$}
        \STATE Pick up $t$-th sub-array $\Ycal_n^k$ in $\Scal_n$
        \STATE Carry out variational E-step to optimize $q(\Mcal_n^k)$ and $q(\Zcal_n^k)$
        \STATE Calculate $\partial g_{k}(\tUcal_n)$ and update $\tUcal_n$ according to Equation \eqref{eq:var_m_tu}.
    \ENDFOR
    \RETURN $\tUcal_n$
    %\REQUIRE $n \geq 0 \vee x \neq 0$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\ours($\{\Scal_1, \ldots, \Scal_N\}$, $\Ucal_0$, $T$, $\eta$, $R$)}
\label{alg:dintucker}
\begin{algorithmic}
\STATE Initialize $\Ucal$ with $\Ucal_0$.
\REPEAT
    \FORALL  {$i \in \{1,\ldots, N\}$ \textbf{parallel} }
        \STATE MAP task $i$: $\tUcal_i=\textrm{SGD}(\Scal_i, T, \eta, \Ucal)$
    \ENDFOR
    \STATE REDUCE task: Aggregate from all MAP results $\{\tUcal_1, \ldots, \tUcal_N\}$ to update $\Ucal$, according to Equation \eqref{eq:var_m_u}.
\UNTIL {$R$ iterations}
\RETURN $\Ucal$
\end{algorithmic}
\end{algorithm}

\subsection{Predicting tensor entries}
Let us denote the training tensor as $\Ycal$ and the learned latent factors as $\Ucal=\{\U^{(1)},\ldots, \U^{(K)}\}$.  To predict the value for a new entry $\bi=\{i_1, \ldots, i_K\}$, we first sample a set of latent factors in each mode. Then we add the $i_1$-th latent factor in $\U^{(1)}$, the $i_2$-th latent factor in $\U^{(2)}$ and so on until all the latent factors corresponding to entry $\bi$ is added into the factors set. We denote the latent factor set as $\Ucal_\xi=\{\U_\xi^{(1)},\ldots,\U_\xi^{(K)}\}$. Then based on the locations of factors in $\Ucal_\xi$, we can extract the sub-array $\Ycal_{\xi}$. Then given $\Ucal_\xi$, we perform the variational E-step as in Equations \eqref{eq:var_e_z} and \eqref{eq:var_e_M} to obtain the posterior distribution of $q(\Mcal_\xi)$. We simply use the posterior mean of $q(\Mcal_\xi)$ for prediction, \ie we use the value of the entry in $\expec{q}{\Mcal_\xi}$ corresponding to the same latent factors as $\bi$ as the prediction result. We can repeat the procedure for server times and take the average prediction value as the final prediction. Moreover, we can predict a batch of test entry values in the same way.

Similar to the learning procedure, our scheme to predict a new tensor entry is  based on much smaller sub-arrays containing that entry. \InfTucker, however, needs to infer the whole latent tensor $q(\Mcal)$ in order to query the specific entry value, which is infeasible for large application.


